Forging Spatial Intelligence: A Roadmap of Multi-Modal Data Pre-Training for Autonomous Systems

The rapid advancement of autonomous systems, including self-driving vehicles and drones, has intensified the need to forge true Spatial Intelligence from multi-modal onboard sensor data. While foundation models excel in single-modal contexts, integrating their capabilities across diverse sensors like cameras and LiDAR to create a unified understanding remains a formidable challenge. This paper presents a comprehensive framework for multi-modal pre-training, identifying the core set of techniques driving progress toward this goal. We dissect the interplay between foundational sensor characteristics and learning strategies, evaluating the role of platform-specific datasets in enabling these advancements. Our central contribution is the formulation of a unified taxonomy for pre-training paradigms: ranging from single-modality baselines to sophisticated unified frameworks that learn holistic representations for advanced tasks like 3D object detection and semantic occupancy prediction. Furthermore, we investigate the integration of textual inputs and occupancy representations to facilitate open-world perception and planning. Finally, we identify critical bottlenecks, such as computational efficiency and model scalability, and propose a roadmap toward general-purpose multi-modal foundation models capable of achieving robust Spatial Intelligence for real-world deployment.

==> tables/benchmark_results/domain_image2lidar.tex <==
\begin{table*}
    \centering
    \renewcommand\tabcolsep{3pt}
    \caption{Comparisons of image-to-LiDAR data pre-training on ScribbleKITTI~\cite{}, RELLIS-3D~\cite{}, SemanticPOSS~\cite{}, SemanticSTF~\cite{}, SynLiDAR~\cite{}, DAPS-3D~\cite{}, Synth4D~\cite{}, and nuScenes-C~\cite{} datasets, respectively.}
    \vspace{-0.25cm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{r|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{20pt}<{\centering}p{20pt}<{\centering}|p{22pt}<{\centering}p{22pt}<{\centering}}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{ScriKITTI}} \vline & \multicolumn{2}{c}{\textbf{RELLIS-3D}} \vline & \multicolumn{2}{c}{\textbf{SemPOSS}} \vline & \multicolumn{2}{c}{\textbf{SemSTF}} \vline & \multicolumn{2}{c}{\textbf{SynLiDAR}} \vline & \multicolumn{2}{c}{\textbf{DAPS-3D}} \vline & \multicolumn{2}{c}{\textbf{Synth4D}} \vline & \multicolumn{2}{c}{\textbf{nuScenes-C}}
    \\
    & \textbf{1\%} & \textbf{10\%} & \textbf{1\%} & \textbf{10\%} & \textbf{Half} & \textbf{Full} & \textbf{Half} & \textbf{Full} & \textbf{1\%} & \textbf{10\%} & \textbf{Half} & \textbf{Full} & \textbf{1\%} & \textbf{10\%} & \textbf{mCE} & \textbf{mRR}
    \\\midrule\midrule
    Random & 23.81 & 47.60 & 38.46 & 53.60 & 46.26 & 54.12 & 48.03 & 48.15 & 19.89 & 44.74 & 74.32 & 79.38 & 20.22 & 66.87 & 112.20 & 72.57
    \\\midrule
    PPKT \cite{liu2021learning} & 36.50 & 51.67 & 49.71 & 54.33 & 50.18 & 56.00 & 50.92 & 54.69 & 37.57 & 46.48 & 78.90 & 84.00 & 61.10 & 62.41 & 105.64 & 75.87
    \\
    SLidR \cite{sautier2022image} & 39.60 & 50.45 & 49.75 & 54.57 & 51.56 & 55.36 & 52.01 & 54.35 & 42.05 & 47.84 & 81.00 & 85.40 & 63.10 & 62.67 & 106.08 & 75.99
    \\
    Seal \cite{liu2024segment} & 40.64 & 52.77 & 51.09 & 55.03 & 53.26 & 56.89 & 53.46 & 55.36 & 43.58 & 49.26 & 81.88 & 85.90 & 64.50 & 66.96 & 92.63 & 83.08
    \\
    SuperFlow \cite{xu20244d} & 42.70 & 54.00 & 52.83 & 55.71 & 54.41 & 57.33 & 54.72 & 56.57 & 44.85 & 51.38 & 82.43 & 86.21 & 65.31 & 69.43 & 91.67 & 83.17 
    \\
    LargeAD \cite{kong2025largead} & 43.45 & 54.62 & 53.31 & 56.62 & 54.47 & 57.11 & 55.14 & 56.89 & 47.12 & 52.82 & 83.31 & 86.21 & 65.33 & 67.12 & 91.75 & 83.61
    \\
    LiMoE \cite{xu2025limoe} & 43.95 & 55.96 & 53.74 & 56.67 & 55.42 & 57.83 & 55.60 & 57.31 & 45.79 & 52.27 & 83.24 & 86.68 & 66.54 & 71.07 & 88.43 & 83.28
    \\
    \bottomrule
\end{tabular}}
\label{table:domain_image2lidar}
\end{table*}
